Model-Free Reinforcement Learning for Asset Allocation

Asset allocation (or portfolio management) is the task of determining how to optimally allocate funds of a finite budget into a range of financial instruments/assets such as stocks. This study investigated the performance of reinforcement learning (RL) when applied to portfolio management using model-free deep RL agents. We trained several RL agents on real-world stock prices to learn how to perform asset allocation. We compared the performance of these RL agents against some baseline agents. We also compared the RL agents among themselves to understand which classes of agents performed better. From our analysis, RL agents can perform the task of portfolio management since they significantly outperformed two of the baseline agents (random allocation and uniform allocation). Four RL agents (A2C, SAC, PPO, and TRPO) outperformed the best baseline, MPT, overall. This shows the abilities of RL agents to uncover more profitable trading strategies. Furthermore, there were no significant performance differences between value-based and policy-based RL agents. Actor-critic agents performed better than other types of agents. Also, on-policy agents performed better than off-policy agents because they are better at policy evaluation and sample efficiency is not a significant problem in portfolio management. This study shows that RL agents can substantially improve asset allocation since they outperform strong baselines. On-policy, actor-critic RL agents showed the most promise based on our analysis.

==> chapters/chapter02.tex <==
\section{Reinforcement Learning}



\subsection{Introduction to Reinforcement Learning}
Reinforcement Learning (RL) is the type of learning guided by a specific objective. An agent learns by interacting with an unknown environment, typically in a trial-and-error way. Whereby RL is an approach to machine intelligence that combines two disciplines to successfully solve problems that neither discipline can address individually \cite{huang_deep_2020}. Due to the development in computing technologies throughout the years, the goals of artificial intelligence (AI) have been a step closer. AI is a programmable machine that tries to mimic the workings of the human brain through machine learning (ML). ML is a sub-field of AI that focuses on the use of data and algorithms to imitate the way that humans learn, gradually improving its accuracy \cite{filos_reinforcement_2019}. There are mainly three categories of ML.

\begin{enumerate}
    \item Supervised learning
    \item Unsupervised learning
    \item Reinforcement learning
\end{enumerate}

The first category of supervised learning is related to learning from a set of training data of labelled examples that are provided by a domain expert who takes the role of the external supervisor in the learning process. The goal is to enable the learning agent with the capability to generalize responses to cases not included in the training set. The second category Unsupervised learning is related to finding hidden patterns and knowledge into a dataset, without any supervision. Finally, Reinforcement Learning (RL) is the type of learning guided by a specific objective. An agent learns by interacting with an unknown environment, typically in a trial-and-error way. This is the most common way of learning for a child, who does something and observes what happens. The agent receives feedback in terms of a reward (or punishment) from the environment; then, it uses this feedback to train itself and collect experience and knowledge about the environment

Reinforcement learning is an orthogonal approach that addresses different, more difficult questions by combining the fields of dynamic programming and supervised learning to yield powerful machine-learning systems. Reinforcement learning appeals to many researchers because of its generality in the possibility of solving problems that have been previously unsolvable.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.5]{RL-illustration.png}
    \caption{Components of a reinforcement learning problem}
    \label{fig:RL components}
\end{figure}

The environment is the world where an agent or software algorithm can interact or move. The input to the environment is an agent’s action $A(t)$ taken in the current state $S(t)$ while the environment output is the next state $S(t+1)$ and reward $R(t+1)$. The environment can be anything that processes and determines an agent’s actions and corresponding consequences (next pair of observations and rewards.)

A state is defined as places, positions in each world/environment where an agent can reach or visit. Also, a state can be the information used to determine what happens next. Formally, a state is a function of history: $S_t= f(H_t)$ \cite{filos_reinforcement_2019}.

The reward function $R(t)$ returns a numerical value that an agent can get for being in a state after taking an action. Rewards tell whether a state is useful or not such that the agent gets a higher reward when moving in useful states and a lower reward when moving in undesirable states \cite{noauthor_reinforcement_2021}. The reward hypothesis states that all goals can be described by the maximization of the expected cumulative reward. $R(t)$ also acts as feedback for an agent which can be positive or negative.

Actions are anything that an agent can imagine or be allowed to do in an environment. For example, in a grid world \cite{gao_framework_2021}, an agent may go left, right, down, up, or can stay in the current state. In a single horizontal line environment, an agent can move left or right. In general, an agent may opt for any action that is available in each scenario.

The agent receives the controlled state of the system and a reward associated with the last state transition. It then calculates a control signal (action) which is sent back to the system. In response, the system makes a transition to a new state and the cycle is repeated. The goal is to learn a way of controlling the system (policy) to maximize the total reward.

A reinforcement learning agent may include one or more of these components:
\begin{itemize}
    \item Policy: A policy guides an agent on which action to choose in each state. It is a mapping from a set of states to a corresponding set of actions. An optimal policy gives long-term optimized rewards that an agent could get in a lifetime. \cite{gao_framework_2021, betancourt_deep_2021}
    \item Value function: It determines how good each state is, or state-action pair. The notion of “how good” here is defined in terms of future rewards that can be expected, or, to be precise, in terms of expected return.
    \item Model: This is the agent’s representation of the environment by predicting what the environment will do next \cite{filos_reinforcement_2019, silver_general_2018}
\end{itemize}

\subsection{Notations}
\input{chapters/chapter02/notation}



\subsection{Reinforcement Learning Algorithms}
Any RL algorithm can be classified as policy-based or value-based or a combination of both i.e. actor-critic method \cite{betancourt_deep_2021} \cref{fig:RL approaches}. The Value-based RL algorithm estimates the optimal value function Q(s,a), this is the maximum value achievable under any policy. Examples of these algorithms include Q-Networks, Q-Learning, Deep Q-Networks (DQN)\cite{li_online_2014, levisauskait_investment_nodate-1, huang_deep_2020}. While the Policy-based RL algorithm searches directly for the optimal policy ($\pi^*$), this is the policy achieving a maximum future reward. Examples of this kind of algorithms include Deep Policy Networks, Policy Gradients, Actor-Critic Algorithm, Asynchronous Advantage Actor-Critic (A3C), Deep DPG, Fictitious Self-Play (FSP). \cite{li_online_2014, gao_framework_2021, noauthor_reinforcement_2021}.etc 

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.35]{RL_algorithm_categorization.png}
    \caption{Summary of approaches in RL based on whether we want to model the value, policy, or the environment}
    \label{fig:RL approaches} \cite{lilianweng_long_2018}
\end{figure}

The above algorithms can also be classified as  model-free algorithms, for example, Q-learning. In model-based RL, an agent can make predictions about different states and corresponding rewards after learning \cite{silver_general_2018, betancourt_deep_2021}. These methods depend on trial and error to update their experience and knowledge about the given environment as they do not have knowledge of the transition model and reward function. They must learn the system dynamics by interacting with the environment many times. Model-based algorithms such as dynamic programming, transition models, and return function. In this algorithm, an agent does not rely on trials instead it exploits an already learned model \cite{betancourt_deep_2021}. 

There are about four common approaches to reinforcement learning:
\begin{enumerate}
    \item Dynamic Programming
    
    This is a two-step process used when the model is fully known. First, policy evaluation is done, and then policy improvement using the Bellman equations.
    
    \item Monte Carlo Methods
    
    Monte-Carlo (MC) methods learn from episodes of raw experience without modeling the environmental dynamics and compute the observed mean return as an approximation of the expected return. This means that learning can only take place after complete episodes.
    
    \item Temporal Difference
    
    Temporal difference methods aim to improve on Monte Carlo methods by learning from incomplete episodes. Sutton \& Barto (2017) describes it as “one idea … central and novel to reinforcement learning” to emphasize its importance. It relies on bootstrapping to carry out value estimation. It can be considered as a combination of dynamic programming and Monte Carlo.

    \item Policy Gradient
    
    While temporal difference methods relied on value estimation to determine the best policy, policy gradient methods rely on policy estimation directly. The policy, $\pi(a|s;\theta)$, is parameterized by $\theta$ and we can use gradient ascent to find the best $\theta$ that produces the highest return. 
    
    Policy learning can be done either in an on-policy or off-policy manner. On-policy methods attempt to evaluate or improve the policy that is used to make decisions. In contrast, off-policy methods evaluate or improve a policy different from that used to generate the data. 
    
    The Tables below shows a grid of some common model-free RL methods based on their learning mechanics

\end{enumerate}

\input{chapters/chapter02/tables_of_model_free_RL_algorithms} \label{RL_Algos_table}

\begin{figure}[p]
    \centering
    \includegraphics[scale=0.5]{Taxonomy-of-RL-Algorithms.png}
    \caption{Taxonomy of Reinforcement learning Algorithms} \cite{harveymachine}
    \label{fig:RL Taxonomy}
\end{figure}

\clearpage

\subsubsection{REINFORCE}
\input{chapters/chapter02/reinforce}

\subsubsection{Actor critic Algorithm(A2C)}
\input{chapters/chapter02/a2c} 

\subsubsection{Soft Actor-Critic Algorithm(SAC)}
\input{chapters/chapter02/sac} 

\subsubsection{Trust Region Policy Optimization (TRPO)}
\input{chapters/chapter02/trpo}

\subsubsection{Proximal Policy Optimization (PPO)}
\input{chapters/chapter02/ppo}

\subsubsection{Deep Deterministic Policy Gradient (DDPG)}
\input{chapters/chapter02/ddpg}

\subsubsection{Twin Delayed Deep Deterministic Policy Gradient (TD3)}
\input{chapters/chapter02/td3}

\subsubsection{Normalized Advantage Function (NAF, Alias - Deep Soft Q- Network (DSQN}
\input{chapters/chapter02/naf}




\section{Machine Learning in Finance}
Machine learning has become increasingly important in the finance industry across several tasks given the volume of data that is available. Figure 1 shows a taxonomy of some of the common applications of machine learning in finance.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=1.0]{ml-in-finance.png}
    \caption{Taxonomy of Common Applications of Machine Learning in Finance}
    \label{fig:ML Taxonomy in Finance}
\end{figure}

For financial tasks, the following classes of machine learning algorithms have been frequently used:

\begin{itemize}
\item Generalized Linear Models: LASSO, Ridge Regression, Elastic Net
\item Tree-based Models: Decision Trees, Random Forest, Boosted Trees
\item Kernel-based Methods: Support Vector Machines
\item Neural-based Models: Multilayer Perceptron, Recurrent Neural Networks, Gated Recurrent Units, Long-Short Term Memory Networks, Generative Adversarial Networks, Deep Autoencoders, \item Deep Belief Networks, Restricted Boltzmann Machines, Deep Reinforcement Learning
Probabilistic Models - Latent Dirichlet Allocation, Naive Bayes

\end{itemize}


The table below shows different research works where the aforementioned models and several others were used, the task that was being performed, and what the input data was.


\input{chapters/chapter02/previous_ml_research_in_AI}

As seen in the table, reinforcement learning has found several applications in stock price prediction, portfolio management/allocation, tax evasion prediction, and trading signal generation among others. In the following paragraphs, we will be providing an overview of several significant works that have been done in the domain of reinforcement learning for portfolio management

In \cite{filos_reinforcement_2019}, a universal model-free reinforcement learning family of agents was introduced. This framework was both memory and computationally efficient because it generalizes across assets and markets regardless of the training universe. Furthermore, the author leveraged pre-training, data augmentation, and simulation to ensure more robust training.

In \cite{gao_framework_2021}, a hierarchical reinforcement learning framework that can handle an arbitrary number of assets and takes into account the transaction fees were proposed. The framework shows good performance on real market data. However, only four stocks were considered making the framework’s ability to deal with large-scale data doubtful. 

In \cite{betancourt_deep_2021}, the authors introduced a more general framework for performing portfolio management on the cryptocurrency market with transaction costs in a universe of dynamic assets (i.e. new assets can be integrated during deployment without extra training or memory). The proposed method had average daily returns of over 24% on the test set.

In \cite{jiang_deep_2017}, an extensible reinforcement learning framework for solving a general portfolio management task was introduced. The framework relies on the Ensemble of Identical Independent Evaluators (EIIE) meta topology which allows for many types of weight-sharing neural networks at the lower level. This framework was tested on the cryptocurrency market and was said to outperform other compared trading algorithms by a distance.

In \cite{hu_deep_2019}, the authors proposed Deep Gated Recurrent Units (GRU) for deep learning and policy gradient for reinforcement learning to search the optimal policy function’s parameters. The GRU models automatically keep track of past states and history while reinforcement learning helps make the portfolio management decisions.

In \cite{huotari_deep_2020}, the authors investigated the portfolio performance of a trading agent based on a convolutional neural network model. The agent’s behavior correlated with an investor's behavior of high risk-taking. Also, the agent outperformed benchmarks but its performance did not statistically differ significantly from the S\&P 500 index.

In \cite{hieu_deep_2020}, the author investigated three state-of-the-art continuous policy gradient algorithms - Deep Deterministic Policy Gradient (DDPG), Generalized Deterministic Policy Gradient (GDPG), and Proximal Policy Optimization (PPO). The author concluded that the former two performed much better than the last one.




==> chapters/chapter02/notation.tex <==
Table \ref{tab:RL Notation} shows a list of RL-related notations.

\begin{table}[H]
    \centering
    \caption{RL Notations \protect \cite{lilianweng_long_2018}}
    \renewcommand*{\arraystretch}{1.4}
    \begin{tabular}{| l | p{0.85\textwidth} | }
    \hline
    \hline
         \textbf{Symbol} & \textbf{Meaning} \\
    \hline
    \hline
    $s \in \mathcal{S}$ & States. \\
    \hline
    $a \in \mathcal{A}$ & Actions. \\
    \hline
    $r \in \mathcal{R}$ & Rewards. \\
    \hline
    $S_t, A_t, R_t$ & State, action, and reward at time step t of one trajectory. \\
    \hline
    $\gamma$ & Discount factor; penalty to uncertainty of future rewards; $0<\gamma \leq 1$. \\
    \hline
    $G_t$ & Return; or discounted future reward; $G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1}$. \\
    \hline
    $P(s', r \vert s, a)$ & Transition probability of getting to the next state $s'$ from the current state $s$ with action $a$ and reward $r$. \\
    \hline
    $\pi(a \vert s)$ & Stochastic policy (agent behavior strategy); $\pi_\theta(.)$ is a policy parameterized by $\theta$. \\
    \hline
    $\mu(s)$ & Deterministic policy; we can also label this as $\pi(s)$, but using a different letter gives better distinction so that we can easily tell when the policy is stochastic or deterministic without further explanation. Either $\pi$ or $\mu$ is what a reinforcement learning algorithm aims to learn. \\
    \hline
    $V(s)$ & State-value function measures the expected return of state $s; V_w(.)$ is a value function parameterized by $w$. \\
    \hline
    $V^\pi(s)$ & The value of state $s$ when we follow a policy 
    $\pi$; $V^\pi (s) = \mathbb{E}_{a\sim \pi} [G_t \vert S_t = s]$. \\
    \hline
    $Q(s, a)$ & Action-value function is similar to $V(s)$, but it assesses the expected return of a pair of state and action $(s, a); Q_w(.)$ is a action value function parameterized by $w$. \\
    \hline
    $Q^\pi(s, a)$ & Similar to $V^\pi(.)$, the value of (state, action) pair when we follow a policy $\pi; Q^\pi(s, a) = \mathbb{E}_{a\sim \pi} [G_t \vert S_t = s, A_t = a]$. \\
    \hline
    $A(s, a)$ & Advantage function, $A(s, a) = Q(s, a) - V(s)$; it can be considered as another version of Q-value with lower variance by taking the state-value off as the baseline. \\
    \hline
    \hline

    \end{tabular}
    \label{tab:RL Notation}
\end{table}

\clearpage


==> chapters/chapter03.tex <==
\section{Gym Environment}
\subsection{Assumptions/Liberties}
The environment takes in the following inputs:
\begin{itemize}
    \item Data
    \item Episode length
    \item Return type: log returns or sharpe ratio
    \item Trading costs: Default = 0.01
    \item Lookback period: Default 64 (3 months)
    \item Retain Cash: Default True
    \item Random Start Position
    \item Seed
    \item Investment
    \item Start date
    \item End date
    \item Exp Constant
    \
\end{itemize}



\subsection{Subsection Title}
Sed metus quam, ultricies vel mi ac, volutpat accumsan nulla. Morbi condimentum consectetur lorem non lobortis. Nam tincidunt ipsum neque, in dignissim velit mattis sed. Aenean laoreet magna erat, nec dictum lacus viverra ut. Duis convallis sapien sed nisl rhoncus aliquam. Nullam sodales quam sed fermentum interdum. Vestibulum vulputate tincidunt ante ultrices elementum. Fusce ex sem, feugiat non metus quis, vehicula eleifend leo. Pellentesque in tellus scelerisque, mollis mi vel, ultricies dolor. Maecenas velit dui, condimentum et finibus ut, vehicula nec erat. Quisque in tempus tortor. Ut ut sem est. Morbi leo magna, molestie ac urna vitae, auctor tristique tellus. Ut sit amet mauris nec metus molestie accumsan vel nec ante.

\subsection{Subsection Title}
Nulla dui orci, commodo sit amet odio non, posuere fermentum lorem. Etiam non lorem in nibh pharetra lacinia vel ut purus. Nullam iaculis porta risus, quis aliquam dui mollis at. Pellentesque tempor convallis dui quis scelerisque. Cras urna arcu, malesuada at ornare sed, tempor nec ipsum. Morbi placerat malesuada dolor. Donec hendrerit ligula ut quam ornare, et pretium ex viverra. Pellentesque eget ipsum eu tellus fringilla vulputate sit amet nec erat. Praesent pretium posuere tellus interdum varius. Aliquam condimentum vel nibh sed lacinia. Fusce dignissim vitae nunc in interdum. Sed sit amet dignissim nunc, ac finibus diam. Proin bibendum turpis vel nulla consequat luctus. Morbi efficitur feugiat accumsan.

\subsection{Subsection Title}
Duis ut est rhoncus, pulvinar turpis eu, volutpat magna. Nam ac felis eleifend, venenatis diam et, consequat nibh. Morbi nec pellentesque libero. Sed diam nibh, vehicula ut lorem sit amet, luctus dictum ex. Praesent non quam ac dolor feugiat gravida. Ut consequat convallis gravida. Proin id suscipit augue. Praesent et turpis in elit pellentesque feugiat vitae a eros. Maecenas eu metus vitae diam interdum sodales vitae et dolor. Proin ipsum sapien, dapibus quis purus vitae, malesuada condimentum sem. Donec mollis commodo lectus, id varius erat auctor non.

\subsection{Subsection Title}
Suspendisse potenti. Donec ut vestibulum est, ultricies eleifend ante. Pellentesque eu libero et nulla sollicitudin pellentesque. Sed rhoncus odio a purus venenatis, ut hendrerit nisi luctus. Mauris consectetur lectus id velit interdum laoreet. Interdum et malesuada fames ac ante ipsum primis in faucibus. Nulla tristique fringilla elit ac congue. Cras felis nunc, tincidunt ut lorem sed, varius volutpat urna. Curabitur sit amet tincidunt nisi. Mauris consequat volutpat dui iaculis suscipit. Quisque faucibus sapien in sapien tempor imperdiet.
